LCQPow -- A Solver for Linear Complementarity Quadratic Programs

In this paper we introduce an open-source software package written in C++ for efficiently finding solutions to quadratic programming problems with linear complementarity constraints. These problems arise in a wide range of applications in engineering and economics, and they are challenging to solve due to their structural violation of standard constraint qualifications, and highly nonconvex, nonsmooth feasible sets. This work extends a previously presented algorithm based on a sequential convex programming approach applied to a standard penalty reformulation. We examine the behavior of local convergence and introduce new algorithmic features. Competitive performance profiles are presented in comparison to state-of-the-art solvers and solution variants in both existing and new benchmarks.

==> chapters/limitations.tex <==

\section{Limitations}

\todo{Should I write about this? Counter Examples}

% TODO: Write about
% 1: Strictly convex functions
% 2: LICQ assumption
% 3: LCQPs (still not the interesting class MPCCs)
% 4: Counter examples: Moritz example with two constraints


%\input{figures/limitations/counter1.svg}

==> chapters/miqp.tex <==

\section{Solving Mixed Integer Quadratic Programs}\label{sec:miqp}
Consider the complementarity constraint
\begin{equation}\label{binary:encoding}
    0 \leq b \perp 1 - b \geq 0
\end{equation}
and note that this encodes a binary variable $b$ with the only feasible points of~\eqref{binary:encoding} being $b = 0$ and $b = 1$. The binary representation of a nonnegative integer value $z \in \Z_{\geq 0}$ is then given by
\begin{subequations}\label{integer:encoding}
    \begin{eqnarray}
        z &=& \sum_{i = 1}^{n_B} 2^{(i-1)} b_i, \\
        0 &\leq& b_i \perp 1 - b_i \geq 0, \quad \mathrm{for}~i \in \{ 1, \dots, n_B\} \label{integer:encoding:bits},
    \end{eqnarray}
\end{subequations}
where $n_B$ denotes the number of bits available in the system. Using this representation one could consider solving \acp{miqp} via a complementarity approach. The constraints in~\eqref{integer:encoding:bits} form a $n_B$-dimensional unit cube, and precisely its vertices represent the nonnegative integer values. A two dimensional illustration is given in~\figref{fig:binary:representation}. Of course, this heuristic only leads to local solutions, however it could be a fast approximation.
\begin{figure}
    \begin{subfigure}[b]{.475\linewidth}
        \includegraphics[width=\linewidth,left]{./figures/MIQP/bin_rep_box_2d.pdf}
        \caption{Penalty level lines and feasible area with binary variables $b_i$ and $b_j$.}
        \label{fig:binary:representation:level:feasible}
    \end{subfigure}%
    \begin{minipage}[b]{.05\linewidth}
        \phantom{~}
    \end{minipage}%
    \begin{subfigure}[b]{.475\linewidth}
        \includegraphics[width=\linewidth,right]{./figures/MIQP/bin_curvature.pdf}
        \caption{Penalty function values including a regularization term centered at $\tfrac{1}{2}$.}
        \label{fig:binary:representation:pen:vals}
    \end{subfigure}
    \caption{Binary penalty function analyzed  . The penalty is minimized in the four corners, which represent the feasible integer numbers, namely $0$, $2^{i-1}$, $2^{j-1}$, and $2^{i-1} + 2^{j-1}$.. The penalty is minimized in the four corners, which represent the feasible integer numbers, namely $0$, $2^{i-1}$, $2^{j-1}$, and $2^{i-1} + 2^{j-1}$.}
    \label{fig:binary:representation}
\end{figure}

Note that the binary complementarity constraint~\eqref{binary:encoding} yields a strictly concave penalty function, centered at $\frac{1}{2}$. Consequently, if the complementarity constraints only consist of binary ones, then the line search is no longer required. Every full step will automatically minimize the merit function along the step direction. In this case the globalization process can be switched off safely. One could consider adding the regularization term $(b-0.5)^2 - 0.25$ for each binary variable $b$. This idea is motivated from the fact that the concave penalty term is maximized at $0.5$, which provides a good initialization for the linearization process. Further, this regularization term does not impact the solution of the original \ac{miqp}, as it vanishes at every feasible point.

We use this heuristic approach to solve a real-world \ac{miqp}. This problem appears as a subproblem within the mixed-integer nonlinear model predictive control task of operating a solar-driven climate system~\cite{Buerger2021Experimental}. The authors solve the problem in three steps, out of which the \ac{miqp} step is of essential expense. The problem has $4388$ optimization variables $4934$ linear constraints and $182$ complementarity constraints. The \solverref solver finds a reasonably good local solution with objective value about $21388$ in roughly $69$ seconds. In comparison, the global solution obtained by the \ac{miqp} solver \gurobi has objective value about $10317$ and was obtained in approximately \todo{how long?} seconds. \figref{fig:miqp:trajectory:results} shows the results of both approaches.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{./figures/MIQP/comparison0.pdf}
    \caption{Comparing the result to solutions obtained via \gurobi.}
    \label{fig:miqp:trajectory:results}
\end{figure}

==> tables/MacMPEC/table_compl.tex <==

\newcommand{\rowspacing}{1.3}
\newcommand{\headerformats}{lrrrrrrr}
\newcommand{\headers}{problem & LCQPow qpOASES & LCQPow OSQP & Gurobi & IPOPT penalty & IPOPT smoothed & IPOPT relaxed & IPOPT NLP\
}

\ra{\rowspacing}
\begin{tabular}{@{}\headerformats @{}}\toprule 
\headers \\ \midrule
bard1 & 1.47e-14 & - & 0 & -2.92e-10 & 1.00e-07 & 1.00e-07 & 1.05e-08\\
bard1m & 1.95e-14 & - & 0 & 0 & 1.00e-07 & 1.00e-07 & 9.59e-09\\
bard2 & 4.65e-14 & 4.74e-14 & 0 & 1.61e-20 & 1.00e-06 & 1.61e-20 & 1.61e-20\\
bilevel2 & 3.30e-14 & 2.59e-07 & 0 & 3.62e-07 & 1.00e-07 & 6.67e-07 & 4.48e-09\\
bilevel2m & 1.07e-07 & 2.69e-07 & 0 & 1.00e-06 & 1.00e-07 & 6.66e-07 & 5.12e-09\\
ex9.2.1 & 9.86e-31 & - & 0 & -2.23e-10 & 1.00e-07 & 1.00e-07 & 1.10e-08\\
ex9.2.2 & 2.89e-07 & 2.89e-07 & 0 & 2.89e-07 & 1.00e-07 & 1.00e-07 & 1.21e-08\\
ex9.2.4 & 4.44e-16 & 4.44e-16 & 0 & 1.03e-10 & 1.00e-07 & 1.00e-07 & 1.01e-08\\
ex9.2.5 & 2.22e-16 & 2.00e-15 & 0 & 0 & 1.00e-07 & 1.00e-07 & 1.13e-08\\
ex9.2.6 & 2.22e-16 & 1.33e-11 & 0 & 3.05e-11 & 1.00e-07 & 1.00e-07 & 5.00e-09\\
ex9.2.7 & 7.40e-31 & - & 0 & -2.23e-10 & 1.00e-07 & 1.00e-07 & 1.10e-08\\
flp2 & 3.55e-15 & 5.33e-15 & -1.78e-15 & 5.00e-07 & 1.00e-06 & 7.18e-07 & 5.03e-09\\
flp4.1 & 7.58e-16 & 7.58e-16 & 0 & -1.22e-12 & 1.00e-07 & -1.22e-12 & -1.22e-12\\
flp4.2 & 7.85e-16 & 8.87e-16 & 0 & -5.78e-12 & 1.00e-07 & -5.78e-12 & -5.78e-12\\
flp4.3 & 8.81e-16 & 8.81e-16 & 0 & -4.84e-13 & 1.00e-07 & -4.86e-13 & -4.84e-13\\
flp4.4 & 8.48e-16 & 8.73e-16 & 0 & -6.04e-12 & 1.00e-07 & -6.04e-12 & -6.04e-12\\
gauvin & -8.88e-16 & 3.11e-15 & 0 & 0 & 1.00e-07 & 1.00e-06 & 1.14e-08\\
hs044.i & 2.00e-15 & - & 2.56e-09 & 2.67e-07 & 1.00e-07 & 6.67e-07 & 1.21e-08\\
jr1 & 0 & 0 & 0 & -4.43e-11 & 1.00e-06 & -4.50e-11 & -1.80e-11\\
jr2 & 1.11e-16 & 1.39e-16 & 0 & -3.39e-11 & 1.00e-06 & 1.00e-07 & 1.01e-08\\
kth2 & -2.22e-16 & -2.22e-16 & 0 & -9.00e-11 & 1.00e-07 & -9.00e-11 & -8.72e-11\\
kth3 & 2.22e-16 & 2.22e-16 & 0 & -6.58e-11 & 1.00e-07 & 1.00e-07 & 1.01e-08\\
liswet1.050 & 5.53e-15 & 4.96e-09 & 6.83e-15 & -3.19e-12 & 1.00e-06 & -3.20e-12 & -3.20e-12\\
liswet1.100 & 3.00e-14 & - & 2.24e-14 & -3.20e-12 & 1.00e-06 & -3.20e-12 & -3.21e-12\\
liswet1.200 & 1.09e-13 & - & -1.44e-03 & -4.18e-12 & 1.00e-06 & -4.05e-12 & -4.18e-12\\
nash1a & 7.55e-25 & 3.55e-15 & 0 & 4.57e-07 & 1.00e-07 & 5.04e-07 & 4.02e-09\\
nash1b & 7.55e-25 & 7.11e-15 & 0 & 4.23e-07 & 1.00e-07 & 5.04e-07 & 4.02e-09\\
nash1c & -7.55e-25 & 3.55e-15 & 0 & 4.18e-07 & 1.00e-07 & 5.04e-07 & 4.04e-09\\
nash1d & 0 & 3.55e-15 & 0 & 4.59e-07 & 1.00e-07 & 5.04e-07 & 4.02e-09\\
nash1e & 7.55e-25 & 7.89e-31 & 0 & 4.61e-07 & 1.00e-07 & 5.04e-07 & 4.02e-09\\
portfl1 & 8.18e-19 & 2.04e-12 & 0 & 1.75e-12 & 1.00e-07 & 1.00e-07 & 1.01e-08\\
portfl2 & 2.16e-20 & 8.33e-13 & 0 & 9.39e-13 & 1.00e-07 & 1.00e-07 & 1.02e-08\\
portfl3 & 6.39e-19 & 3.94e-08 & 0 & 3.94e-08 & 1.00e-07 & 1.00e-07 & 1.02e-08\\
portfl4 & 3.78e-17 & 4.32e-12 & 0 & 1.53e-12 & 1.00e-07 & 1.00e-07 & 1.01e-08\\
portfl6 & 4.00e-17 & 5.50e-12 & 0 & 7.28e-13 & 1.00e-06 & 1.00e-07 & 1.02e-08\\
qpec1 & 2.22e-16 & 2.22e-16 & 0 & 0 & 1.00e-07 & 0 & 0\\
qpec2 & 3.47e-08 & 3.47e-08 & 0 & 5.55e-07 & 1.00e-07 & 1.00e-07 & 1.16e-09\\
scholtes3 & 2.22e-16 & 2.22e-16 & 0 & 0 & 1.00e-07 & 1.00e-07 & 1.01e-08\\
sl1 & 2.22e-17 & 3.36e-10 & -9.37e-16 & 1.89e-07 & 1.00e-07 & 1.94e-07 & 5.00e-09\\
\bottomrule
\end{tabular}


==> tables/MacMPEC/table_objectives.tex <==

\newcommand{\rowspacing}{1.3}
\newcommand{\headerformats}{lrrrrrrrr}
\newcommand{\headers}{problem & best known & LCQPow qpOASES & LCQPow OSQP & Gurobi & IPOPT pen & IPOPT sm & IPOPT rel & IPOPT NLP\
}

\small{
\ra{\rowspacing}
\begin{tabular}{@{}\headerformats@{}}\toprule 
\headers \\ \midrule
bard1 & 17 & 25 & - & 17 & 17 & 17 & 25 & 17\\
bard1m & 17 & 25 & - & 17 & 17 & 17 & 25 & 17\\
bard2 & -6598 & -6598 & -6598 & -6598 & -6598 & -6.60e+03 & -6598 & -6598\\
bilevel2 & -6600 & -6600 & -6600 & -6600 & -6600 & -6600 & -6600 & -6600\\
bilevel2m & -6600 & -6600 & -6600 & -6600 & -6600 & -6600 & -6600 & -6600\\
ex9.2.1 & 17 & 25 & - & 17 & 17 & 17 & 25 & 17\\
ex9.2.2 & 100 & 1.00e+02 & 1.00e+02 & 100 & 1.00e+02 & 1.00e+02 & 1.00e+02 & 1.00e+02\\
ex9.2.4 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01\\
ex9.2.5 & 5 & 9 & 9 & 5 & 9 & 5 & 9 & 9.80e+00\\
ex9.2.6 & -1 & -1 & -1 & -1 & -1 & -1.00e+00 & -1 & -1\\
ex9.2.7 & 17 & 25 & - & 17 & 17 & 17 & 25 & 17\\
flp2 & 0 & 2.34e-12 & 2.34e-12 & 2.34e-12 & 2.34e-12 & 8.87e-12 & 2.34e-12 & 7.60e-12\\
flp4.1 & 0 & -1.55e-15 & -1.55e-15 & 0 & -2.70e-09 & 7.02e-06 & -2.70e-09 & -2.70e-09\\
flp4.2 & 0 & -2.22e-16 & -1.11e-15 & 0 & -5.40e-09 & 6.32e-06 & -5.40e-09 & -5.40e-09\\
flp4.3 & 0 & 1.55e-15 & 1.55e-15 & 0 & -6.30e-09 & 7.90e-06 & -6.30e-09 & -6.30e-09\\
flp4.4 & 0 & 6.66e-16 & -2.22e-15 & 0 & -9.00e-09 & 1.18e-05 & -9.00e-09 & -9.00e-09\\
gauvin & 20 & 20 & 20 & 20 & 20 & 325 & 20 & 20\\
hs044.i & 1.56e+01 & 6.25e-06 & - & 6.25e-06 & 6.25e-06 & 1.56e+01 & 6.25e-06 & 1.56e+01\\
jr1 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01\\
jr2 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01\\
kth2 & 0 & -2.22e-16 & -2.22e-16 & 0 & -9.00e-11 & 1.00e-07 & -9.00e-11 & -8.72e-11\\
kth3 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01\\
liswet1.050 & 1.40e-02 & 1.40e-02 & 1.40e-02 & 1.40e-02 & 1.40e-02 & 1.30e-01 & 1.40e-02 & 1.40e-02\\
liswet1.100 & 1.37e-02 & 1.37e-02 & - & 1.37e-02 & 1.37e-02 & 2.40e-01 & 1.37e-02 & 1.37e-02\\
liswet1.200 & 1.70e-02 & 1.70e-02 & - & 3.38e-02 & 1.70e-02 & 4.75e-01 & 1.70e-02 & 1.70e-02\\
nash1a & 7.89e-30 & 5.20e-12 & 5.20e-12 & 4.71e-12 & 1.27e-11 & 4.71e-12 & 5.59e-12 & 4.71e-12\\
nash1b & 7.89e-30 & 5.20e-12 & 5.20e-12 & 4.71e-12 & 1.25e-11 & 4.71e-12 & 5.59e-12 & 4.71e-12\\
nash1c & 7.89e-30 & 5.20e-12 & 5.20e-12 & 4.71e-12 & 1.25e-11 & 4.71e-12 & 5.59e-12 & 4.71e-12\\
nash1d & 7.89e-30 & 5.20e-12 & 5.20e-12 & 4.71e-12 & 1.27e-11 & 4.71e-12 & 5.59e-12 & 4.71e-12\\
nash1e & 7.89e-30 & 5.20e-12 & 5.20e-12 & 4.71e-12 & 5.55e-12 & 4.71e-12 & 5.59e-12 & 4.71e-12\\
portfl1 & 1.50e-05 & 2.04e-02 & 2.04e-02 & 2.04e-02 & 2.04e-02 & 2.06e-02 & 2.04e-02 & 2.04e-02\\
portfl2 & 1.46e-05 & 2.78e-02 & 2.78e-02 & 2.79e-02 & 2.78e-02 & 2.97e-02 & 2.78e-02 & 2.78e-02\\
portfl3 & 6.27e-06 & 2.28e-02 & 2.27e-02 & 2.31e-02 & 2.27e-02 & 2.27e-02 & 2.27e-02 & 2.28e-02\\
portfl4 & 2.18e-06 & 2.05e-02 & 2.05e-02 & 2.21e-02 & 2.05e-02 & 2.06e-02 & 2.05e-02 & 2.05e-02\\
portfl6 & 2.36e-06 & 2.40e-02 & 2.40e-02 & 2.16e-01 & 2.40e-02 & 2.46e-02 & 2.40e-02 & 2.40e-02\\
qpec1 & 80 & 80 & 80 & 80 & 80 & 8.00e+01 & 80 & 80\\
qpec2 & 45 & 4.50e+01 & 4.50e+01 & 45 & 4.50e+01 & 4.50e+01 & 4.50e+01 & 4.50e+01\\
scholtes3 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 5.00e-01 & 1.00e+00\\
sl1 & 1.00e-04 & 1.00e-04 & 1.00e-04 & 1.00e-04 & 1.00e-04 & 1.00e-04 & 1.00e-04 & 1.00e-04\\
\bottomrule
\end{tabular}
}

==> tables/MacMPEC/table_timings.tex <==

\newcommand{\rowspacing}{1.3}
\newcommand{\headerformats}{lrrrrrrr}
\newcommand{\headers}{problem & LCQPow qpOASES & LCQPow OSQP & Gurobi & IPOPT penalty & IPOPT smoothed & IPOPT relaxed & IPOPT NLP\
}

\ra{\rowspacing}
\begin{tabular}{@{}\headerformats @{}}\toprule 
\headers \\ \midrule
bard1 & 2.02e-04 & - & 2.95e-03 & 3.16e-01 & 2.07e-01 & 2.75e-01 & 3.09e-02\\
bard1m & 1.91e-04 & - & 1.83e-03 & 3.73e-01 & 3.50e-01 & 3.28e-01 & 5.24e-02\\
bard2 & 3.11e-04 & 1.57e-04 & 1.81e-03 & 3.62e-02 & 3.90e-01 & 1.38e-01 & 1.38e-01\\
bilevel2 & 1.06e-03 & 1.49e-03 & 1.71e-03 & 1.14e-01 & 5.03e-01 & 2.93e-01 & 1.34e-01\\
bilevel2m & 6.29e-04 & 1.39e-03 & 1.55e-03 & 9.53e-02 & 6.67e-01 & 5.20e-01 & 2.02e-01\\
ex9.2.1 & 2.41e-04 & - & 3.12e-03 & 3.08e-01 & 1.79e-01 & 4.59e-01 & 1.11e-01\\
ex9.2.2 & 4.79e-04 & 1.94e-03 & 1.38e-03 & 6.39e-01 & 1.67e-01 & 2.55e-01 & 4.07e-02\\
ex9.2.4 & 2.63e-04 & 5.06e-04 & 1.07e-03 & 2.77e-01 & 2.07e-01 & 2.15e-01 & 7.60e-02\\
ex9.2.5 & 3.38e-04 & 1.25e-03 & 1.67e-03 & 3.77e-01 & 1.37e-01 & 3.17e-01 & 5.22e-02\\
ex9.2.6 & 4.18e-04 & 2.93e-03 & 2.18e-03 & 6.71e-01 & 2.36e-01 & 3.12e-01 & 7.91e-02\\
ex9.2.7 & 2.53e-04 & - & 2.23e-03 & 3.03e-01 & 1.87e-01 & 2.49e-01 & 6.08e-02\\
flp2 & 1.19e-04 & 1.44e-03 & 1.15e-03 & 5.56e-02 & 2.16e-01 & 1.40e-01 & 7.07e-02\\
flp4.1 & 1.38e-02 & 3.00e-03 & 8.30e-03 & 1.88e-02 & 3.73e-01 & 4.76e-02 & 2.29e-02\\
flp4.2 & 3.93e-02 & 7.30e-03 & 2.52e-02 & 3.35e-02 & 6.72e-01 & 1.00e-01 & 3.56e-02\\
flp4.3 & 6.94e-02 & 1.41e-02 & 9.92e-02 & 9.12e-02 & 7.88e-01 & 2.31e-01 & 1.40e-01\\
flp4.4 & 1.97e-01 & 3.19e-02 & 9.98e-02 & 7.57e-02 & 2.23e+00 & 3.42e-01 & 1.20e-01\\
gauvin & 1.99e-04 & 6.56e-04 & 1.65e-03 & 3.41e-01 & 2.51e-01 & 1.75e-01 & 3.37e-02\\
hs044.i & 2.84e-04 & - & 1.82e-03 & 1.60e-01 & 2.81e-01 & 3.03e-01 & 6.99e-02\\
jr1 & 6.52e-05 & 6.40e-05 & 1.01e-03 & 1.21e-02 & 1.07e-01 & 2.87e-02 & 2.83e-02\\
jr2 & 1.57e-04 & 3.03e-04 & 1.13e-03 & 2.39e-01 & 1.04e-01 & 1.84e-01 & 8.48e-02\\
kth2 & 6.31e-05 & 5.52e-05 & 1.82e-04 & 1.26e-02 & 1.09e-01 & 2.88e-02 & 3.77e-02\\
kth3 & 1.57e-04 & 2.89e-04 & 1.14e-03 & 2.21e-01 & 9.96e-02 & 1.65e-01 & 3.69e-02\\
liswet1.050 & 7.00e-02 & 2.56e-02 & 1.33e-02 & 7.73e-02 & 1.56e+00 & 2.25e-01 & 9.91e-02\\
liswet1.100 & 5.79e-01 & - & 3.21e-02 & 1.61e-01 & 2.76e+00 & 4.49e-01 & 1.81e-01\\
liswet1.200 & 6.82e+00 & - & 1.21e-01 & 3.32e-01 & 5.11e+00 & 9.83e-01 & 3.83e-01\\
nash1a & 1.41e-04 & 4.03e-03 & 1.07e-03 & 8.17e-02 & 1.52e-01 & 2.07e-01 & 2.90e-02\\
nash1b & 1.43e-04 & 2.20e-03 & 1.10e-03 & 7.74e-02 & 1.52e-01 & 1.71e-01 & 6.51e-02\\
nash1c & 1.53e-04 & 2.18e-03 & 1.05e-03 & 9.57e-02 & 1.56e-01 & 1.95e-01 & 2.39e-02\\
nash1d & 1.58e-04 & 2.13e-03 & 9.98e-04 & 7.86e-02 & 1.54e-01 & 1.79e-01 & 6.43e-02\\
nash1e & 1.40e-04 & 2.08e-03 & 1.06e-03 & 5.53e-02 & 1.47e-01 & 1.79e-01 & 4.18e-02\\
portfl1 & 8.21e-03 & 1.13e-02 & 4.88e-02 & 8.45e-01 & 4.49e-01 & 4.64e-01 & 8.14e-02\\
portfl2 & 1.16e-02 & 2.42e-02 & 4.19e-02 & 8.97e-01 & 4.74e-01 & 4.63e-01 & 8.04e-02\\
portfl3 & 9.58e-03 & 3.04e-02 & 5.18e-02 & 8.85e-01 & 4.09e-01 & 4.70e-01 & 1.59e-01\\
portfl4 & 8.60e-03 & 1.08e-02 & 4.69e-02 & 8.52e-01 & 4.41e-01 & 4.53e-01 & 8.03e-02\\
portfl6 & 9.25e-03 & 1.29e-02 & 4.34e-02 & 8.99e-01 & 3.60e-01 & 4.80e-01 & 1.39e-01\\
qpec1 & 5.15e-04 & 1.80e-04 & 5.06e-03 & 1.21e-02 & 1.57e-01 & 2.69e-02 & 1.69e-02\\
qpec2 & 7.11e-03 & 2.40e-03 & 7.32e-03 & 4.47e-01 & 1.53e-01 & 2.01e-01 & 4.20e-02\\
scholtes3 & 1.93e-04 & 3.24e-04 & 1.56e-03 & 3.18e-01 & 2.60e-01 & 2.02e-01 & 3.66e-02\\
sl1 & 1.28e-04 & 2.33e-04 & 7.31e-04 & 7.02e-02 & 6.82e-01 & 1.70e-01 & 1.28e-01\\
\bottomrule
\end{tabular}


==> widebar.tex <==
% From https://tex.stackexchange.com/questions/16337/can-i-get-a-widebar-without-using-the-mathabx-package

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother
